Neuromorphic Graph Anomaly Detection via Adaptive STDP and Spiking Graph Neural Networks

Anomaly detection in dynamic networks is critical for applications from cybersecurity to industrial monitoring, yet existing methods face challenges in energy efficiency, temporal precision, and adaptability. This paper introduces ASTDP-GAD, a novel Adaptive Spiking Temporal Dynamics Plasticity framework for Graph Anomaly Detection that integrates spiking graph neural networks with STDP learning for energy-efficient neuromorphic detection in dynamic networks. Our framework unifies spiking neural computation, STDP learning, and graph-based anomaly detection through the following key innovations: temporal spike graph encoding with adaptive Leaky Integrate-and-Fire (LIF) dynamics; LIF-based graph attention with lateral inhibition; event-driven hypergraph memory with STDP-inspired prototype updates; spike rate contrast pooling based on spiking irregularity; adaptive STDP layers capturing causal temporal relationships; and multi-scale temporal convolution with multi-factor anomaly fusion. Theoretical analysis provides rigorous guarantees: spike encoding preserves input information with resolution scaling linearly in simulation steps and hidden dimension; LIFGAT approximates any continuous attention function; hypergraph memory converges to optimal prototypes; contrast pooling achieves provable anomaly selection bounds; STDP learning converges stably; and multi-factor fusion produces calibrated scores with up to $5\times$ variance reduction. Extensive experiments on nine datasets on both dynamic and static graphs demonstrate superior anomaly detection accuracy while maintaining biological plausibility and energy efficiency for neuromorphic deployment.

==> section/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes
    \item[] Justification: The abstract and introduction (Section~\ref{sec:introduction}) clearly state that ASTDP-GAD integrates spiking neural mechanisms, STDP, and adaptive graph learning for neuromorphic anomaly detection. Main claims include theoretical guarantees (Section~\ref{sec:theoretical}) and empirical results showing state-of-the-art performance across nine datasets (Section~\ref{sec:experiments}, Tables~\ref{tab:ablation_study}, \ref{tab:complexity}). Limitations are discussed in Section~\ref{sec:discussion} (\ref{subsec:limitations} and~\ref{subsec:future_work}).

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes
    \item[] Justification: Limitations are thoroughly discussed in Section~\ref{sec:discussion} (Limitations and Failure Cases subsection), including: (1) $O(T N H^2)$ complexity for deep architectures, (2) moderate supervision requirements (60\% training data for 95\% performance), (3) heavy-tailed error distributions potentially underestimating rare anomaly risks, and (4) dataset-dependent hyperparameter optimisation. 

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:theoretical} provides complete theoretical analysis with five theorems (Theorems~\ref{thm:spike_encoding}--\ref{thm:fusion_calibration}), each including clear assumptions, proof sketches in the main text, and references to complete proofs in Appendix~\ref{sec:theoretical}. Lemma statements and assumptions are explicitly numbered and cross-referenced.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:experiments} provides a complete experimental setup, including data splits (30/60/80\% training ratios), hyperparameters (default values in Table~\ref{tab:sensitivity_analysis}), optimisation details (AdamW with a learning rate of $2^{-4}$ and weight decay of $5^{-4}$), and model architecture specifications. Appendix~\ref{sec:hyperparameters} provides exhaustive hyperparameter search ranges that provide exact environment configuration.
    
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo
    \item[] Justification: All datasets used (DBLP, Tmall, Patent, BlogCatalog, T-Social, Flickr, Yelp, T-Finance, Amazon) are publicly available with proper citations (Section~\ref{sec:preprocessing}, Table~\ref{tab:datasets}). The code is proprietary at this time. An anonymised zip file containing core inference code, model checkpoints, and reproduction instructions would be provided when the source code is released for verification.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:experiments} specifies all training and test details: data splits, training minibatch size for GPU and CPU(1024/4096), optimiser (Adam, lr=$10^{-3}$, weight decay=$10^{-5}$), training epochs (200 with early stopping), hyperparameter selection (grid search with validation), and evaluation metrics (Macro-F1, AUC-ROC, and AUC-PR in Appendix~\ref{sec:metrics}). Appendix~\ref{sec:hyperparameters} provides complete parameter tables.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: All main results (ablation study, sensitivity analysis, baseline comparisons) report mean values over five independent runs with different random seeds. Section~\ref{sec:experiments} specifies that standard deviations are reported in Table~\ref{tab:sensitivity_analysis} and error analysis in Figure~\ref{fig:case_study}. Statistical significance tests (paired t-test, $p<0.05$) are referenced in the ablation analysis.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:complexity} and Table~\ref{tab:complexity} provide detailed compute resource specifications: NVIDIA V100 32GB GPU, mini-batch size 1024, training time per epoch (36.7 ms on DBLP, 1,345 ms on Patent), inference latency (0.13 ms/node on DBLP, 0.39 ms/node on Patent), and GPU memory (198 MB training, 167 MB inference). Total compute for all experiments was approximately 500 GPU hours.
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes
    \item[] Justification: The research conforms to the NeurIPS Code of Ethics. All datasets are publicly available and used in accordance with their licenses. No human subjects were involved. The research focuses on anomaly detection for cybersecurity and fraud prevention, with ethical considerations discussed in Section~\ref{sec:discussion} (Broader Impact subsection).

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:discussion} (Broader Impact and Implications for Networked Systems subsections) discusses both positive societal impacts (energy-efficient edge deployment for IoT security, cybersecurity monitoring, financial fraud detection, social network moderation) and potential negative impacts (privacy concerns in surveillance applications, dual-use risks for adversarial evasion). Mitigation strategies (gated deployment, uncertainty-aware thresholding) are proposed.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA
    \item[] Justification: The paper does not release pre-trained models or datasets that pose high risk for misuse. All datasets are standard public benchmarks. The method is defensive (anomaly detection) rather than generative, and no dual-use model checkpoints are released. If deployed, safeguards would be application-dependent (e.g., false positive rate thresholds).

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes
    \item[] Justification: Section~\ref{sec:preprocessing} properly cites all datasets with their original papers. Licenses are summarised: DBLP (Academic Free License), Tmall (research use), Patent (public domain), BlogCatalog (research use), T-Social (research use), Flickr (CC BY 2.0), Yelp (research use), T-Finance (research use), Amazon (MIT). Baseline method citations include original papers and code repositories where applicable.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo
    \item[] Justification: The paper does not release new datasets or pretrained models. The anonymised code provided in supplemental material is for reproducibility verification only and is not a formal asset release. No new benchmarks or datasets are introduced.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects. All experiments use publicly available graph benchmark datasets.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA
    \item[] Justification: No human subjects research was conducted. IRB approval is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA
    \item[] Justification: LLMs were not used as a core component of the ASTDP-GAD methodology. LLMs may have been used for writing assistance, but this does not impact the core methodology, scientific rigour, or originality of the research.

\end{enumerate}
